Robust Recovery via Implicit Bias of Discrepant Learning Rates for Double Over-parameterization

Recent advances have shown that implicit bias of gradient descent on over-parameterized models enables the recovery of low-rank matrices from linear measurements, even with no prior knowledge on the intrinsic rank. In contrast, for robust low-rank matrix recovery from grossly corrupted measurements, over-parameterization leads to overfitting without prior knowledge on both the intrinsic rank and sparsity of corruption. This paper shows that with a double over-parameterization for both the low-rank matrix and sparse corruption, gradient descent with discrepant learning rates provably recovers the underlying matrix even without prior knowledge on neither rank of the matrix nor sparsity of the corruption. We further extend our approach for the robust recovery of natural images by over-parameterizing images with deep convolutional networks. Experiments show that our method handles different test images and varying corruption levels with a single learning pipeline where the network width and termination conditions do not need to be adjusted on a case-by-case basis. Underlying the success is again the implicit bias with discrepant learning rates on different over-parameterized parameters, which may bear on broader applications.

==> qq_defs.tex <==



\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography

\usepackage{graphicx,amsmath,amsfonts,amscd,amssymb,bm,url,color,latexsym}

\usepackage[inline]{enumitem}
\usepackage{mwe}
%\usepackage{subfigure}
%\usepackage{subfig}
\usepackage{subcaption}
%\usepackage{bbm}
%\usepackage{bm}
%\usepackage{microtype}
\setlength{\captionmargin}{30pt}
\usepackage{algorithm,algorithmicx}
\usepackage{algpseudocode}
%\usepackage{hyperref}
\usepackage[nameinlink]{cleveref}
%\usepackage{verbatim}
\usepackage{framed}
\usepackage{comment}
\usepackage{wrapfig}
\usepackage{tikz}
\usepackage{pgfplots}
%\usepackage[margin=0.95in]{geometry}
%\usepackage{tikz}
%\usepackage{multirow}
%\usepackage{cleveref}

\usepackage{tablefootnote}
\usepackage{tcolorbox}
%\usepackage{pifont}
\usepackage{authblk}
%\usepackage[margin=0.95in]{geometry}

\providecommand{\keywords}[1]{\textbf{\textit{Index terms---}} #1}


% pagebreak for long equations
%\allowdisplaybreaks

\hypersetup{
    colorlinks=true,%
    citecolor=blue,%
    filecolor=blue,%
    linkcolor=blue,%
    urlcolor=blue
}
\usepackage[toc, page]{appendix}
%%%%%%%%%%%%%%
\renewcommand\floatpagefraction{.95}
\renewcommand\topfraction{.95}
\renewcommand\bottomfraction{.95}
\renewcommand\textfraction{.05}
\setcounter{totalnumber}{50}
\setcounter{topnumber}{50}
\setcounter{bottomnumber}{50}
%%%%%%%%%%%%%%
%--------------
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}


\newtheorem{assumption}[theorem]{Assumption}


\newcommand{\indep}{\rotatebox[origin=c]{90}{$\models$}}

\renewcommand{\mathbf}{\boldsymbol}

\newcommand{\conv}{\circledast}
\newcommand{\mb}{\mathbf}
\newcommand{\mc}{\mathcal}
\newcommand{\mf}{\mathfrak}
\newcommand{\md}{\mathds}
\newcommand{\bb}{\mathbb}
\newcommand{\magnitude}[1]{ \left| #1 \right| }
\newcommand{\set}[1]{\left\{ #1 \right\}}
\newcommand{\condset}[2]{ \left\{ #1 \;\middle|\; #2 \right\} }

\newcommand{\wc}{\widecheck}

\newcommand{\reals}{\bb R}
\newcommand{\proj}{\mathrm{proj}}
\newcommand{\E}{\mathbb{E}}

\newcommand{\eps}{\varepsilon}
\newcommand{\R}{\reals}
\newcommand{\Cp}{\bb C}
\newcommand{\Z}{\bb Z}
\newcommand{\N}{\bb N}
\newcommand{\Sp}{\bb S}
\newcommand{\Ba}{\bb B}
\newcommand{\indicator}[1]{\mathbbm 1_{#1}}
\renewcommand{\P}{\mathbb{P}}

\newcommand{ \Brac }[1]{\left\lbrace #1 \right\rbrace}
\newcommand{ \brac }[1]{\left[ #1 \right]}
\newcommand{ \paren }[1]{ \left( #1 \right) }
\newcommand{\col}{\mathrm{col}}


% to declare new operator
% \DeclareMathOperator{\xxx}{xxx}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\poly}{poly}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\trace}{tr}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\vect}{vec}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\Hess}{Hess}
\DeclareMathOperator{\mini}{minimize}
\DeclareMathOperator{\maxi}{maximize}
\DeclareMathOperator{\st}{subject\; to}

%% Other definitions


\newcommand{\wh}{\widehat}
\newcommand{\wt}{\widetilde}
\newcommand{\ol}{\overline}



\newcommand{\norm}[2]{\left\| #1 \right\|_{#2}}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\innerprod}[2]{\left\langle #1,  #2 \right\rangle}
\newcommand{\prob}[1]{\bb P\left[ #1 \right]}
\newcommand{\expect}[1]{\bb E\left[ #1 \right]}
\newcommand{\function}[2]{#1 \left(#2\right)}
\newcommand{\integral}[4]{\int_{#1}^{#2}\; #3\; #4}


\newcommand{ \vphi }[1]{ \varphi( #1 ) }
\newcommand{ \vphiT }[1]{ \varphi_{\mathrm{T}}( #1 ) }
\newcommand{ \vphiDL }[1]{ \varphi_{\mathrm{DL}}( #1 ) }
\newcommand{ \vphiCDL }[1]{ \varphi_{\mathrm{CDL}}( #1 ) }
\newcommand{ \TvphiCDL }[1]{ \ol{\varphi}_{\mathrm{CDL}}( #1 ) }
\newcommand{ \HvphiCDL }[1]{ \wh{\varphi}_{\mathrm{CDL}}( #1 ) }
\newcommand{ \vphiICA }[1]{ \varphi_{\mathrm{ICA}}( #1 ) }

\newcommand{ \init }[1]{{\mathbf #1}_{\mathrm{init}}}

\newcommand{\qq}[1]{{\color{blue}{\bf Qing: #1}}}
\newcommand{\sz}[1]{{\color{blue}{\bf Simon: #1}}}
\newcommand{\zz}[1]{{\color{purple}{#1}}}
\newcommand{\yz}[1]{{\color{blue}{\bf Yuqian: #1}}}
\newcommand{\td}[1]{{\color{magenta}{\bf TODO: #1}}}
\newcommand{\edit}[1]{{\color{black}{#1}}}
\newcommand{\edited}[1]{{\color{black}{#1}}}

%\numberwithin{equation}{section}

%\def \endprf{\hfill {\vrule height6pt width6pt depth0pt}\medskip}
\newenvironment{proof}{\noindent {\bf Proof} }{\endprf\par}

\newcommand{\qed}{{\unskip\nobreak\hfil\penalty50\hskip2em\vadjust{}
           \nobreak\hfil$\Box$\parfillskip=0pt\finalhyphendemerits=0\par}}


\newcommand{\mr}{\mathrm}
\newcommand{\inprod}[2]{\langle#1,#2\rangle}
\newcommand{\parans}[1]{\left(#1\right)}


\newcommand{\res}[2]{\mb \iota_{ #1 \rightarrow #2  }}
\newcommand{\shift}[2]{{\mathrm{s}_{#2}}\left[#1\right]}
\newcommand{\Shift}[2]{{\wh{\mathrm{s}}_{#2}}\left[#1\right]}

==> sections/broad_impacts.tex <==
\section*{Broader Impact}

Robust learning of structured signals from high-dimensional data has a wide range of applications, including imaging processing, computer vision, recommender systems, generative models and many more. In this work, we presented a new type of practical methods and provided improved understandings of solving these problems via over-parameterized models. 
In particular, our method exploits the implicit bias introduced by the learning algorithm, with the underlying driving force being the intrinsic structure of the data itself rather than human handcrafting. 
Such a design methodology helps to eliminate human bias in the design process, hence provides the basis for developing truly fair machine learning systems. 


% Since the result in , this work does not present any foreseeable societal consequence.


% ========

% \textbf{Example}: GNNs (and hence GNNExplainer) could be applied to a wide range of applications, including computer vision, natural language processing, recommender systems, traffic prediction, generative models and many more (Zhou et al 2019, Wu et al 2019). Our research could be used to provide explanations for GNNs in these applications, improving understanding of individual decisions, as well as the underlying models.

% While there will be important impacts resulting from the use of GNNs in general, here we focus on the impact of using our tool to provide explanations for such systems There are many benefits to using such a tool, such as increasing the transparency in decision-critical applications. This can help mitigate fairness, privacy and safety risks — see the introduction of the paper for more details. The potential risks of increasing explainability have typically received less attention. These include: (i) the risk of automation bias, i.e. an undue trust in models (see e.g. PAI 2019), (ii) if the use of explanations means systems may now be used by those with lower levels of domain or ML expertise, this could increase the risk of the model or its outputs being used incorrectly, (iii) if explanations are only used during the development phase, and the model is retrained over time, changing its behaviour, this could again lead to a false sense of security.

% We see opportunities for research applying GNNExplainer to beneficial purposes, such as investigating whether GNNExplainer could improve algorithmic fairness. To mitigate the risks associated with using generated explanations, we encourage research to understand the impacts of using GNNExplainer in particular real-world scenarios. In these scenarios, do users understand the explanations given, and act accordingly, not falling prey to automation bias? Does use of the system improve or diminish domain expertise over time?



\begin{ack}
Chong would like to thank Yaodong Yu and Ryan Chan for the helpful discussions. 
% Use unnumbered first level headings for the acknowledgments. All acknowledgments
% go at the end of the paper before the list of references. Moreover, you are required to declare 
% funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work). 
% More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2020/PaperInformation/FundingDisclosure}.


% Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to autmoatically hide this section in the anonymized submission.
\end{ack}

==> sections/insights.tex <==

First, let us build up some intuitions from a simple linear regression problem.

We use linear regression to illustrate the key properties of step sizes  used in gradient descent  in over-parameterized nonlinear learning. In this case, given data matrix $\mX\in\R^{m\times n}$ and labels $\vy\in\R^m$, the linear regression model amounts to the minimizing the least-squares loss
\e
\min_{\vtheta\in\R^n} f(\vtheta) = \frac{1}{2}\norm{\mX\vtheta - \vy}{2}^2.
\label{eq:lr}\ee
Starting from initialization $\vtheta_0\in\R^n$, gradient descent involves the following update
\e
\vtheta_{k+1} = \vtheta_k - \eta \mX^\T (\mX\vtheta_k - \vy).
\ee
Consider the over-parameterized case where $m\le n$ and the matrix $\mX$ has full row rank such that the global minimum of the loss is 0. Let $\calN(\mX)$ and $\calR(\mX^\T)$ denote the null space and row space of $\mX$, respectively. Since \eqref{eq:lr} is underdetermined, it has infinite number of solution and any of its global minimum belongs to
\e
\calG: = \{\vtheta^\dagger + \ve: \vtheta^\dagger = \mX^\T(\mX\mX^\T)^{-1}\vy, \ \ve \in \calN(\mX)\},
\label{eq:global-lr}\ee
where $\vtheta^\dagger$ has the smallest energy. Note that
\[
\mX\vtheta_{k+1} - \vy = \parans{\mId -\eta \mX\mX^\T}\parans{\mX\vtheta_k - \vy}, 
\]
which implies $\norm{\mX\vtheta_{k+1} - \vy}{}\le \norm{\mId -\eta \mX\mX^\T}{}\norm{\mX\vtheta_k - \vy}{}$. Thus, gradient descent converges to a global minimum as long as $\eta < \norm{\mX\mX^\T}{}$. Let $\vtheta^*$ be the point that gradient descent converges to. To further characterize $\vtheta^*$, denoted by $\calP_{\calR(\mX^\T)}$ and $\calP_{\calN(\mX)}$ the projections onto the null space and the row space of $\mX$, respectively. Since $\calP_{\calR(\mX^\T)} (\vtheta^*) =  \vtheta^\dagger$ and $\calP_{\calN(\mX)}(\vtheta^*) = \calP_{\calN(\mX)}(\vtheta_0)$, we conclude that if $\calP_{\calN(\mX)}(\vtheta_0) = \vzero$ (such as $\vtheta_0 = \vzero$), $\vtheta^* =\vtheta^\dagger$ which is the optimal solution to the following problem
\e \min_{\vtheta\in\R^n} \frac{1}{2}\norm{\vtheta}{2}^2, \quad \st \ \mX\vtheta = \vy.
\label{eq:lr-min-norm}\ee

Thus, gradient descent finds the optimal solution to \eqref{eq:lr-min-norm} if the initialization satisfies $\calP_{\calN(\mX)}(\vtheta_0) = \vzero$, such as $\vtheta_0 = \vzero$.

\paragraph{Different step sizes} We now consider gradient descent with different step sizes for each parameter as
\e
\vtheta_{k+1} = \vtheta_k - \eta \mW \mX^\T (\mX\vtheta_k - \vy),
\label{eq:weighted-gd-lr}\ee
where $\mW$ is an $n\times n$ diagonal matrix with positive diagonals $w_i, i\in[n]$. Here $\eta w_i$ can be viewed as the step size for $\theta_i$. Similarly, note that
\[
\mX\vtheta_{k+1} - \vy = \parans{\mId -\eta \mX\mW\mX^\T}\parans{\mX\vtheta_k - \vy}, 
\]
which implies $\norm{\mX\vtheta_{k+1} - \vy}{}\le \norm{\mId -\eta \mX\mW\mX^\T}{}\norm{\mX\vtheta_k - \vy}{}$. Thus, gradient descent converges to a global minimum as long as $\eta < \norm{\mX\mW\mX^\T}{}$. Let $\wt\vtheta^*$ be the point that gradient descent converges to. Since  $\calP_{\calN(\mX)}(\vtheta^*) = \calP_{\calN(\mX)}(\vtheta_0)$ and $\calP_{\calR(\mX^\T)} (\wt\vtheta^*) =  \wt\vtheta^\dagger$, where $\wt\vtheta^\dagger = \mW\mX^\T(\mX\mW\mX^\T)^{-1}\vy$, we conclude that if $\calP_{\calN(\mX)}(\vtheta_0) = \vzero$ (such as $\vtheta_0 = \vzero$), $\wt\vtheta^* =\wt\vtheta^\dagger$ which is the optimal solution to the following problem
\e
\min_{\vtheta\in\R^n} \frac{1}{2}\norm{\mW^{-1/2 }\vtheta}{2}^2, \quad \st \ \mX\vtheta = \vy.
\label{eq:lr-min-weighted-norm}\ee

Thus, gradient descent with different step sizes \eqref{eq:weighted-gd-lr} finds the optimal solution to \eqref{eq:lr-min-weighted-norm} if the initialization satisfies $\calP_{\calN(\mX)}(\vtheta_0) = \vzero$, such as $\vtheta_0 = \vzero$.
